Bridging the Gap Between Multi-Step and One-Shot Trajectory Prediction via Self-Supervision

Accurate vehicle trajectory prediction is an unsolved problem in autonomous driving with various open research questions. State-of-the-art approaches regress trajectories either in a one-shot or step-wise manner. Although one-shot approaches are usually preferred for their simplicity, they relinquish powerful self-supervision schemes that can be constructed by chaining multiple time-steps. We address this issue by proposing a middle-ground where multiple trajectory segments are chained together. Our proposed Multi-Branch Self-Supervised Predictor receives additional training on new predictions starting at intermediate future segments. In addition, the model 'imagines' the latent context and 'predicts the past' while combining multi-modal trajectories in a tree-like manner. We deliberately keep aspects such as interaction and environment modeling simplistic and nevertheless achieve competitive results on the INTERACTION dataset. Furthermore, we investigate the sparsely explored uncertainty estimation of deterministic predictors. We find positive correlations between the prediction error and two proposed metrics, which might pave way for determining prediction confidence.

==> poster/ablation_table/chapters/results.tex <==


\begin{table}[t!]
	\centering
	\smallskip
\input{tables/component_ablation.tex}

\end{table}



==> poster/ablation_table/setup/acronyms.tex <==
\begin{acronym}
\acro{GPU}{Graphics Processing Units}
\acro{DNN}{Deep Neural Networks}
\acro{CNN}{Convolutional Neural Network}
\acro{RNN}{Recurrent Neural Networks}
\acro{GNN}{Graph Neural Networks}
\acro{GAT}{Graph Attention Networks}
\acro{GCN}{Graph Convolutional Networks}
\acro{GRU}{Gated Recurrent Unit}
\acro{LSTM}{Long Short-Term Memory}
\acro{KF}{Kalman Filters}
\acro{BEV}{Bird's Eye View}
\acro{GAN}{Generative Adversarial Networks}
\acro{MTP}{Multi-Modal Trajectory Prediction}
\acro{MLP}{Multilayer Perceptron}
\acro{MAE}{Mean Absolute Error}
\acro{MSE}{Mean Squared Error}
\acro{ADE}{Average Displacement Error}
\acro{FDE}{Final Displacement Error}
\acro{minADE}{Minimum Average Displacement Error}
\acro{minFDE}{Minimum Final Displacement Error}
\acro{DKM}{Deep Kinematic Models}
\acro{FF-ASP}{Feed-Forward Action-Space Predictor}
\acro{SS-ASP}{Self-Supervised Action-Space Predictor}
\acro{VAE}{Variational Autoencoders}
\acro{CVAE}{Conditional Variational Autoencoder}
\acro{AV}{autonomous vehicle}
\acro{MHA}{Multi-Head Attention}
\acro{SAN}{Scene Anchor Networks}
\acro{MB-SS-ASP}{Multi-Branch Self-Supervised Action-Space Predictor}
\acro{AD}{Autonomous Driving}
\acro{DL}{Deep Learning}
\acro{RL}{Reinforcement Learning}
\acro{MR}{Miss Rate}
\acro{IL}{Imitation Learning}
\acro{MDP}{Markov Decision Process}
\acro{POMDP}{Partially Observable Markov Decision Process}
\acro{RSSM}{Recurrent State Space Models}
\end{acronym}

\hyphenation{mo-de-lab-le know-ledge}
\hyphenation{back-pro-pa-ga-tion}
\hyphenation{re-pre-sen-ting}
\hyphenation{re-gu-la-ri-zer}
\hyphenation{bo-ttle-neck}
\hyphenation{ex-pli-cit-ly}
\hyphenation{an-ti-ci-pate}
\hyphenation{con-sis-ting}
\hyphenation{mar-gi-na-lize}
\hyphenation{me-thods}
\hyphenation{co-ver-age}
\hyphenation{INTERACTION}
\hyphenation{VectorNet}
\hyphenation{mul-ti-ple}
\hyphenation{mo-del}
\hyphenation{mo-dels}

\DeclareMathOperator{\sgn}{sgn}


==> poster/ablation_table/setup/packages.tex <==
% The following packages can be found on http:\\www.ctan.org
%\usepackage{graphics} % for pdf, bitmapped graphics files
%\usepackage{epsfig} % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed

% MATH
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{mathtools}
\usepackage{siunitx}

% TABLES
\usepackage[table,xcdraw]{xcolor}
\usepackage{graphicx}
\usepackage{tabularx,booktabs}
\newcolumntype{Y}{>{\centering\arraybackslash}X}

% MISC
\usepackage{todonotes}
\usepackage[nolist]{acronym}
%\usepackage[para]{footmisc} % footnotes in-line
\usepackage{flushend}
\usepackage[font=small]{caption}
\usepackage[font=small]{subcaption}

% matrix column separation with vertical lines
\makeatletter
\renewcommand*\env@matrix[1][*\c@MaxMatrixCols c]{%
	\hskip -\arraycolsep
	\let\@ifnextchar\new@ifnextchar
	\array{#1}}
\makeatother

%%% citation hyperlinks, must be last
\makeatletter
\let\NAT@parse\undefined
\makeatother

%%%

%%% to show papercept margin limits
%\usepackage[
%showframe,
%top=19.1mm,
%bottom=19.1mm,
%inner=19.1mm,
%outer=19.1mm,
%]{geometry}


%%%% TikZ
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{fadings}
\usetikzlibrary{patterns}
\usetikzlibrary{shadows.blur}
\usetikzlibrary{shapes}
\tikzset{
	vertex/.style={circle,draw,minimum size=2.5em},
	edge/.style={->,> = latex'}
}

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

==> poster/ablation_table/tables/component_ablation.tex <==
\begin{tabularx}{0.5\textwidth}{c *{6}{Y}}
	\toprule
	& & & & & \multicolumn{2}{c}{inD}  \\
	\cmidrule(l){6-7}
	Model & Self-Sup. & Multi-seg. & Multi-branch & Context agg. & min-ADE$_9$ & min-FDE$_9$\\
	\midrule
	FF-ASP [1] & \xmark & \xmark & \xmark & \xmark & 0.22 & 0.56 \\
	SS-ASP [1] & \cmark & \xmark & \xmark & \xmark & 0.19 & 0.50 \\
	Multi-seg. SS-ASP & \cmark & \cmark & \xmark & \xmark & 0.20 & 0.52 \\
	Multi-branch* SS-ASP& \cmark & \cmark & \cmark & \xmark & 0.17 & 0.45 \\
	Multi-branch SS-ASP& \cmark & \cmark & \cmark & \cmark & \textbf{0.17} & \textbf{0.43} \\
	\bottomrule
\end{tabularx}
